Text-Video Retrieval via Variational Multi-Modal Hypergraph Networks

Text-video retrieval is a challenging task that aims to identify relevant videos given textual queries. Compared to conventional textual retrieval, the main obstacle for text-video retrieval is the semantic gap between the textual nature of queries and the visual richness of video content. Previous works primarily focus on aligning the query and the video by finely aggregating word-frame matching signals. Inspired by the human cognitive process of modularly judging the relevance between text and video, the judgment needs high-order matching signal due to the consecutive and complex nature of video contents. In this paper, we propose chunk-level text-video matching, where the query chunks are extracted to describe a specific retrieval unit, and the video chunks are segmented into distinct clips from videos. We formulate the chunk-level matching as n-ary correlations modeling between words of the query and frames of the video and introduce a multi-modal hypergraph for n-ary correlation modeling. By representing textual units and video frames as nodes and using hyperedges to depict their relationships, a multi-modal hypergraph is constructed. In this way, the query and the video can be aligned in a high-order semantic space. In addition, to enhance the model's generalization ability, the extracted features are fed into a variational inference component for computation, obtaining the variational representation under the Gaussian distribution. The incorporation of hypergraphs and variational inference allows our model to capture complex, n-ary interactions among textual and visual contents. Experimental results demonstrate that our proposed method achieves state-of-the-art performance on the text-video retrieval task.

==> del.tex <==
% The motivation behind using the reconstruction loss and KL divergence loss is to ensure that the predicted node representations are close to the actual node representations, and that the predicted distributions are similar to a standard Gaussian.
% The reconstruction loss measures the difference between the predicted node representations and the actual node representations.
% The reconstruction loss $\mathcal{L}_{\text{rec}}$ measures the difference between the predicted node representations and the actual node representations. It is defined as the mean squared error (MSE) between the predicted mean vectors $\boldsymbol{\mu}_{i}$ and the true mean vectors $\mathbf{h}_{i}$, and the MSE between the predicted variance vectors $\boldsymbol{\sigma}_{i}$ and the true variance vectors $\boldsymbol{\tau}_{i}$:
% \begin{equation}
% \mathcal{L}_{\text{rec}}=\frac{1}{n}\sum_{i=1}^{n} \left(|\mathbf{h}_{i}-\boldsymbol{\mu}_{i}|^2+|\boldsymbol{\tau}_{i}-\boldsymbol{\sigma}_{i}|^2\right),
% \end{equation}
% where $n$ is the number of nodes.


% The KL divergence loss measures the difference between the predicted Gaussian distributions and a standard Gaussian distribution.
% The KL divergence loss $\mathcal{L}_{\text{kl}}$ measures the difference between the predicted Gaussian distributions and a standard Gaussian distribution. It is defined as:
% \begin{equation}
% \mathcal{L}_{\text{kl}}=\frac{1}{n}\sum_{i=1}^{n} D_{\text{KL}}(\mathcal{N}(\boldsymbol{\mu}_{i}, \text{diag}(\boldsymbol{\sigma}_{i}^2)) | \mathcal{N}(0, \mathbf{I})),
% \end{equation}
% where $D_{\text{KL}}$ is the Kullback-Leibler divergence and $\mathcal{N}(\mu, \Sigma)$ is the multivariate Gaussian distribution with mean $\mu$ and covariance matrix $\Sigma$.




% The HAN model integrates the variational approach into hypergraph learning, enabling it to model the uncertainty of node representations through Gaussian distributions. This approach allows the model to capture the inherent uncertainty in the data and improves its robustness in handling noisy and incomplete information. Additionally, by using a hypergraph instead of a traditional graph, UMHAN can capture higher-order correlations and interactions among modalities.


% The Variational Hypergraph Attention Networks model has several advantages over traditional hypergraph models. Firstly, it can capture complex correlations among different modalities and has the ability to handle missing data. Secondly, by modeling node representations as Gaussian distributions, it can better capture the uncertainty inherent in real-world data. Finally, by using variational inference, it can learn more robust and accurate node representations.


==> text.tex <==
We propose a multi-modal relation extraction model that constructs a hypergraph including an image and its three objects, as well as the head and tail entities. The hypergraph is constructed using the following equations:

\begin{equation}
\begin{aligned}
x=\delta\left(\sum_{r \in \mathcal{R}} \sum_{e_j \in \mathcal{E}i} \frac{1}{\bar{D}{r, j j}} \boldsymbol{e}_j^l \bar{W}_r^l+x_i^l \bar{W}^l\right),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
x^{w}=\left[x^{I} | x^{{I}{aux1}}\left|x^{{I}{aux2}}\right| x^{{I}_{aux3}}\left|x^{h}\right| x^{t}\right],
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
E^{W}=\operatorname{LeakyReLU}\left(W^{W} \cdot x^{w}\right),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
E^{V}=\operatorname{LeakyReLU}\left(W^{I} \cdot \left[x^{I}\left|x^{{I}{aux1}}\right| x^{{I}{aux2}} | x^{{I}_{aux3}}\right]\right),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
E^{T}=\operatorname{LeakyReLU}\left(W^{T} \cdot \left[x^{h} | x^{t}\right]\right),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
E^{cross}=\operatorname{Normalization}\left(\left([x^{h};x^{t}]\cdot(x^{w})^{T}\right) \cdot x^{w}\right),
\end{aligned}
\end{equation}

where $x$ represents a node, $E$ represents a hyperedge, $x^{w}$ contains $x^{I}$ for the image, $x^{{I}{aux1}}$ for the first object in the image, $x^{{I}{aux2}}$ for the second object in the image, $x^{{I}_{aux3}}$ for the third object in the image, $x^{h}$ for the head entity, and $x^{t}$ for the tail entity. The hyperedges include $E^{V}$ for image hyperedges, $E^{T}$ for text hyperedges, $E^{W}$ for global information hyperedges, and $E^{cross}$ for hyperedges connecting the head or tail entities with the image. The hypergraph is then processed by a HGNN uncertainty model.

Our proposed model incorporates multi-modal information to improve the accuracy of relation extraction. Specifically, the model constructs a hypergraph that includes both image and text information, and utilizes a HGNN uncertainty model to extract relationships between the entities. The hypergraph is constructed using equations that allow for the integration of multiple modalities, including image and text, and the resulting hypergraph is processed by the HGNN to extract the relationships between the entities. The use of the HGNN allows for the modeling of uncertainty, which is particularly important in the context of relation extraction where the existence of relationships between entities may not be clear-cut.

The hypergraph is constructed by representing each entity as a node and connecting them with hyperedges that incorporate information from multiple modalities. Specifically, the hyperedges include $E^{V}$ for image information, $E^{T}$ for text information, $E^{W}$ for global information, and $E^{cross}$ for the relationship between the entities and the image information. The nodes and hyperedges are represented by vectors, and the hyperedges are constructed using equations that allow for the combination of the different modalities.

The HGNN uncertainty model is then applied to the hypergraph to extract relationships between the entities. The model utilizes a LeakyReLU activation function and normalization to ensure the stability of the model during training. Specifically, the model applies the LeakyReLU function to the output of the hypergraph and then normalizes the resulting vectors.

Overall, our proposed multi-modal relation extraction model is a powerful tool for extracting relationships between entities from multiple modalities, and the use of the HGNN uncertainty model allows for the modeling of uncertainty in the relationship extraction process.


The HGNN uncertainty model is applied to the constructed hypergraph to extract relationships between the entities. The model can be formulated as follows:

\begin{equation}
\begin{aligned}
h_{i}^{k+1} &= \sigma\left(\sum_{j\in N(i)}\alpha_{ij}^{k} W^{k} h_{j}^{k}\right)\
\alpha_{ij}^{k}&=\frac{\exp(\beta\cdot f_{ij}^{k})}{\sum_{l\in N(i)}\exp(\beta\cdot f_{il}^{k})}\
f_{ij}^{k}&=h_{i}^{k}\cdot W^{k}\cdot h_{j}^{k}
\end{aligned}
\end{equation}

where $h_{i}^{k}$ is the representation of node $i$ at layer $k$, $W^{k}$ is the learnable weight matrix at layer $k$, $\sigma$ is the activation function, $N(i)$ is the set of neighbors of node $i$, $\alpha_{ij}^{k}$ is the attention weight between node $i$ and its neighbor $j$ at layer $k$, $f_{ij}^{k}$ is the feature importance between node $i$ and its neighbor $j$ at layer $k$, and $\beta$ is a temperature parameter that controls the sharpness of the attention distribution. The final output of the model is a probability distribution over the possible relationships between the head and tail entities.
